Quantization and Semiclassics

This course is aimed at graduate students in physics in mathematics and designed to give a comprehensive introduction to Weyl quantization and semiclassics via Egorov's theorem. Chapter 2 gives a quick overview of classical and quantum mechanics on R^d. Some mathematical preliminaries concerning Hilbert space theory, operator theory and tempered distributions are detailed in Chapters 3-5. Weyl quantization and semiclassics are the content of Chapters 6 and 7. Finally, an application of Weyl calculus to Born-Oppenheimer systems is discussed in Chapter 8.

==> chapters/chapter_09.tex <==
\chapter{Magnetic Weyl calculus (optional)} % (fold)
\label{mag_weyl_calculus}


\section{Quantization of magnetic systems: two ansätze} % (fold)
\label{mag_weyl_calculus:two_paths}

% section quantization_of_magnetic_systems_two_possibilities (end)


\section{Magnetic Weyl quantization} % (fold)
\label{mag_weyl_calculus:magnetic_weyl_quantization}

% section magnetic_weyl_quantization (end)


\section{Magnetic Egorov theorem} % (fold)
\label{mag_weyl_calculus:magnetic_egorov_theorem}

% section magnetic_egorov_theorem (end)



% chapter magnetic_weyl_calculus (end)
